Embodied Question Answering in Photorealistic Environments with Point Cloud Perception

To help bridge the gap between internet vision-style problems and the goal of vision for embodied perception we instantiate a large-scale navigation task -- Embodied Question Answering [1] in photo-realistic environments (Matterport 3D). We thoroughly study navigation policies that utilize 3D point clouds, RGB images, or their combination. Our analysis of these models reveals several key findings. We find that two seemingly naive navigation baselines, forward-only and random, are strong navigators and challenging to outperform, due to the specific choice of the evaluation setting presented by [1]. We find a novel loss-weighting scheme we call Inflection Weighting to be important when training recurrent models for navigation with behavior cloning and are able to out perform the baselines with this technique. We find that point clouds provide a richer signal than RGB images for learning obstacle avoidance, motivating the use (and continued study) of 3D deep learning models for embodied navigation.

==> sections/main/intro.tex <==
\vspace{sectionReduceTop}
\section{Introduction}
\vspace{sectionReduceBot}

For AI agents to harmoniously assist humans in every day activities, they need to be equipped with visual perception, natural language understanding and efficient navigation of novel and realistic environments. While each of these problems has seen tremendous progress in recent years, the advancement of autonomous agents has been slower. Recently, new efforts on building embodied agents for semantic navigation~\cite{gupta_cvpr17, house3d, zhu2017target, zhu2017iccv}, language grounding~\cite{chaplot2017gated, mattersim, hermann2017grounded} and question answering~\cite{embodiedqa, iqa2018} have emerged. However, the lack of diverse and real datasets necessitates the use of synthetic environments which drastically differ from the real world. As a result, the transfer of agents trained on synthetic data to real robotic applications remains an open problem and exploring ways to bridge this gap has drawn the attention of the research community.  

Perception is crucial for real embodied agents. Undoubtedly, modern visual recognition has witnessed significant improvements thanks to the recent advances of deep visual representations~\cite{krizhevsky_nips12, simonyan_iclr15, he_cvpr16}. Commonly, recognition models are trained and tested on well composed data sources, such as images or videos taken by users~\cite{Deng09imagenet, mscoco}. However, for general purpose autonomous agents, access to this form of well framed, object centric visual inputs is not straightforward. Furthermore, for these agents to successfully accomplish their goal, such datasets are inadequate. For example, a house robot needs to enhance its object- and scene-centric perception with free, actionable space prediction and semantic correlations that will result in the correct sequence of primitive actions (\eg turn right, go forward) leading to its goal. These concepts are neither present nor annotated in modern benchmarks, rendering most datasets and supervised learning paradigms tailored for traditional visual recognition tasks (\eg object detection, semantic segmentation) insufficient. 

Moreover, most visual recognition models rely on 2D visual inputs, \eg RGB frames. While such inputs are popular thanks to the easy access to commercial cameras, they hinder autonomous agents, which take actions in the 3D space. With the advent of depth sensing cameras, new input modalities have been introduced, including RGB-D~\cite{} and point clouds~\cite{}. In the deep learning era, effective models have been developed for the tasks of object recognition and segmentation from such input sources~\cite{gupta2014learning, qi2017pointnet}. These input modalities pose new challenges when learning visual representations, including the design of new and more suitable model architectures, and large dataset collection efforts. The impact of these new data modalities has been shown for many robotic tasks~\cite{}. \todo{add more citations}

In this work, we explore the use of point cloud representations for the task of embodied question answering. We train embodied agents that act on point cloud representations of their egocentric view at each time step. For completeness, the input to the agent consists of a set of $(x,y,z)$ points and the corresponding RGB value. We exploit the recent advances on 3D understanding by adopting the PointNet architecture~\cite{qi2017pointnet} and train it to recognize objects from the agent's first person views. At each time step, the output of the our model is used to predict the next primitive action from the agent's current location towards the goal. Contrary to prior work on embodied question answering performed on synthetic environments~\cite{embodiedqa, iqa2018}, we train and test our agents on realistic scenes from Matterport 3D~\cite{Matterport3D}. With the use of point clouds and realistic indoor scenes, our work brings embodied agents trained on simulation one step closer to real autonomous robots equipped with 2.5D RGBD cameras. 

Our dataset consists of .... Our experiments show that ... \todo{Say something about the data and the experimental results}


\begin{itemize}

\item Modern compute vision (specifically internet vision) has scene a large amount of success.

\item The dominate paradigm in this age is that we collect and annotate a large,
  static dataset (ImageNet, COCO, PASCAL) from the internet to train a CNN.
  Typically, the CNN is trained for
  classification and then fine-tuned for its final task, such as detection or segmentation.

\item  Concurrently, we have begun maturing our deep architectures that
  operate directly on point-clouds (PointNet, A-SCN, SplatNet).  These architectures are also trained
  and evaluated on static datasets with tasks such as
  classification, semantic segmentation, object detection.

\item  However, there is a long history of work arguing that the role of perception is
  \emph{for} action.


\item To address this (\ew{maybe a gross overstatement, but I like the flow....})
  , several new tasks have been explored in the broad space of
  Embodied Agents (EQA, IQA, VLN, ....).  These tasks use a 3D environment and an agent
  that perceives the world from 2D RGB images.

\item However, real robots currently used by academia and industry alike have multi-modal
  perceptual inputs from 2.5D \rgbd cameras (examples of common platforms).  Information
    from a 2.5D \rgbd camera is naturally represented by a point-cloud.

\item  There another benefit to using point-clouds: easier collection of datasets.  Current 3D
    environments from real data either make use of complicated meshing algorithms (Matterport3D,
    Surreal's SIGGRAPH paper?)
    or utilized neural networks to fill in missing information (Gibson)
    in order to create photorealistic RGB images from an arbitrary viewpoint.
    Both of these techniques
    are computationally cost and require time-consuming, human assisted, data-collection.

\item Point-clouds are a direct output of SLAM systems.  There is a rich literature on automated,
  exploratory SLAM systems \cite{shen_irca11}

\item 2.5D \rgbd as input has not been explored in the Embodied Agent literature

\item In this work, we compare and contrast the impact of the perception modalities (a CNN trained on RGB
  images or a PointNet architecture trained on point-clouds) on an embodied task -- specifically,
    Embodied Question Answering in the Matterport3D environment.

\item As a byproduct of this exploration, we also present the first photorealistic evaluation
  of an embodied agent in the Matterport3D environment.

\end{itemize}


==> sections/main/intro_v2.tex <==
\section{Introduction}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/teaser.pdf}
    \caption{As in \eqa \cite{embodiedqa}, our agent is spawned in a novel environment and tasked with answering a question about that environment.
    We explore the agent's ability to perceive its environment through point clouds, RGB images, or a combination of the two in order to navigate the environment and answering the question.}
    \label{fig:teaser}
\end{figure}

Imagine walking up to a home robot and asking
\myquote{Hey -- can you go check if my laptop is on my desk? And if so, bring it to me.}
It is clear that in order to be successful, such a robot would need a range of artificial intelligence (AI) skills --
visual perception (to recognize objects, scenes, obstacles),
language understanding (to translate questions and instructions into actions),
and
navigation of potentially novel environments (to move and find things in a changing environment).

The focus of this work is perception for such embodied agents.
While there has been significant progress in the computer vision community
thanks to recent advances in deep visual representations~\cite{krizhevsky_nips12, simonyan_iclr15, he_cvpr16},
we believe there is a growing disconnect between \textbf{\emph{internet vision}} and \textbf{\emph{embodied vision}}.
The focus of the former is recognition in images and videos on datasets typically curated from the internet~\cite{Deng09imagenet, mscoco, antol_iccv15}.
The focus of the latter is perception to enable action by an embodied agent in an environment (\eg a robot).
We focus on two specific points of disconnect:

\begin{enumerate}[leftmargin=*]
\item \textbf{Passive vs Active Vision.}
Internet vision models are trained and tested on passive datasets that often exhibit
framing biases (from users who decide to capture and upload the content) and curation biases
(from researchers who collect the dataset) \cite{agrawal_emnlp16, goyal_cvpr17, torralba2011unbiased}.
For embodied vision, what is needed are not the well-framed object-centric visual inputs typically found in
these datasets, rather \emph{photo-realistic environments} annotated with semantics and free-space where
an agent may learn about the consequence of its actions on its visual input.
A number of recent works have begun studying goal-driven perception-based navigation tasks~\cite{gupta_cvpr17, house3d, zhu2017target, zhu2017iccv,chaplot2017gated, mattersim, hermann2017grounded, embodiedqa, iqa2018}
in such environments. However, most are based
in synthetic
non-perceptually-realistic environments
(on SUNCG~\cite{song_cvpr17} or Unity 3D models~\cite{juliani2018unity}) that drastically differ from the real world and thus,
may not generalize;
indeed, the transfer of agents trained on synthetic data to real robotic applications remains an open problem.

\item \textbf{2D vs 3D Perception.}
Internet vision models are predominantly based on 2D visual inputs, \ie RGB frames. While RGB datasets
are understandably popular thanks to ubiquity of such cameras, it is worth stepping back and asking
-- \emph{why must an embodied agent navigating in 3D environments be handicapped to perceive
with a single RGB camera?}
There is a rich history of depth-sensing cameras in robotic platforms \cite{huang2017visual, zeng2018robotic,
AAMAS17-Zhang}, however, little work
on end-to-end-trained embodied agents that directly perceive in 3D. %
\end{enumerate}




In this work, we address both these points of disconnect -- by instantiating a large-scale navigation
task in photo-realistic environments from Matterport 3D~\cite{Matterport3D} \emph{and}
developing an end-to-end trainable model -- from raw 3D point-clouds to goal-driven navigation policies.

The starting point for our work is the recently proposed task of
Embodied Question Answering (EmbodiedQA)~\cite{embodiedqa} -- where an agent is spawned
at a random location in a novel environment (\eg a house) and asked to answer a question
(\myquote{What color is the car in the garage?}).
In order to succeed, the agent needs to navigate from egocentric vision alone (without an environment map), locate the entity in question (\myquote{car in the garage}),
and respond with the correct answer (\eg \myquote{orange}).


Our primary experimental contribution is that
we generalize EmbodiedQA from the synthetic SUNCG scenes~\cite{song_cvpr17} as studied
by Das~\etal~\cite{embodiedqa} to the photorealistic 3D reconstructions from Matterport 3D~\cite{Matterport3D}
using the MINOS simulator~\cite{savva2017minos}. Specifically, we introduce the \mpeqa dataset,
consisting of 1136 questions and answers grounded in 83 environments. %
In a manner similar to \cite{embodiedqa}, our questions are generated from functional programs operating
on the annotations (objects, rooms, and their relationships) provided in Matterport 3D.
A subtle but important difference between MP3D
and SUNCG is that MP3D objects annotations do not include human names of colors of objects. Since mapping
RGB values to human perceived color names is still a challenging open problem \cite{barron2017fast},
we collect annotations for color names of objects used in our \mpeqa dataset.
The Matterport 3D dataset provides significantly more challenging environments for our
agent to learn to navigate within due to the increased amount of variation.

\newcommand\myeq{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily def}}}{=}}}

Our primary conceptual contribution is the
study of point cloud representations for the EmbodiedQA task in \mpeqa.
Specifically, we leverage the recently proposed PointNet architecture~\cite{qi2017pointnet} and modify it to
compute an \emph{embedding for the point cloud} in the agent's field of view --
a mapping $f$ from an unordered set of points $\{(x_m,y_m,z_m,R_m,G_m,B_m)\}_{m=1}^M \in \mathcal{P}$ to a vector space, \ie $f: \mathcal{P} \longrightarrow \RF^d$.
The network that computes these embeddings is pre-trained on three auxiliary 3D perception tasks
-- semantic labeling of 3D points, color auto-encoding, and depth auto-encoding -- which primes these
embeddings to serve as the basis for 3D navigation. %
Our recurrent neural network (RNN) based navigation model receives
these point-cloud embeddings at each time-stamp,
and is trained via imitation learning (behavior cloning) of expert trajectories automatically
extracted from MINOS free-space annotations.

Our primary technical contribution is the introduction of novel scheme for class-balanced training in behavior cloning when following shortest paths.  We find this scheme to be crucial for generalization from behavior cloning validation accuracy to navigation.

To the best of our knowledge, this is the first work to explore end-to-end-trainable 3D perception
for goal-driven navigation in photo-realistic environments.
With the use of point clouds and realistic indoor scenes,
our work lays the groundwork for tighter connection between embodied vision and goal-driven navigation,
provides a testbed for benchmarking 3D perception models,
and hopefully
brings embodied agents trained on simulation one step closer to real autonomous robots
equipped with 2.5D \rgbd cameras




==> sections/main/pointnet.tex <==
In this work, we apply \pointnet to the \eqa task. \pointnet allows
our agent to perceive its environment directly from \rgbd images.  This gives the agent two main
advantages compared to prior work 1) the agent has an intrinsic knowledge of 3D and 2) it perceives the world
via a format native to readily available consumer grade \rgbd cameras.

Utilizing \rgbd image also provides us a distinct advantage in \matterport.  In VLN
(Anderson et al.) they restrict the agent to only discrete camera locations, which greatly limits the agent's
ability to explore its environment.
While in MINOS they utilize the provided mesh, which does not provide realistic RGB images.
However, \matterport does provide high quality \rgbd images and alignment.  Operating directly on the
\rgbd images greatly alleviates the two drawbacks of these prior works and allows continuous navigation with
realistic sensor data in \matterport.

PointNets are a class of Deep Neural Networks that operate directly on \rgbd data and utilize pointclouds
(an unordered set of$\{X, Y, Z, R, G, B\}$ tuples).  This is done by constructing a symmetric function
(order-invariant) that selects keypoints from the pointcloud and projects them into a high dimensional space.
\pointnet introduces a hierarchical approach to this task.

